PANDA: Architecture-Level Power Evaluation by Unifying Analytical and Machine Learning Solutions

Power efficiency is a critical design objective in modern microprocessor design. To evaluate the impact of architectural-level design decisions, an accurate yet efficient architecture-level power model is desired. However, widely adopted data-independent analytical power models like McPAT and Wattch have been criticized for their unreliable accuracy. While some machine learning (ML) methods have been proposed for architecture-level power modeling, they rely on sufficient known designs for training and perform poorly when the number of available designs is limited, which is typically the case in realistic scenarios. In this work, we derive a general formulation that unifies existing architecture-level power models. Based on the formulation, we propose PANDA, an innovative architecture-level solution that combines the advantages of analytical and ML power models. It achieves unprecedented high accuracy on unknown new designs even when there are very limited designs for training, which is a common challenge in practice. Besides being an excellent power model, it can predict area, performance, and energy accurately. PANDA further supports power prediction for unknown new technology nodes. In our experiments, besides validating the superior performance and the wide range of functionalities of PANDA, we also propose an application scenario, where PANDA proves to identify high-performance design configurations given a power constraint.

==> BackupBib/bibibi.tex <==


@inproceedings{xie2018routenet,
  title={{RouteNet}: Routability prediction for mixed-size designs using convolutional neural network},
  author={Xie, Zhiyao and Huang, Yu-Hung and Fang, Guan-Qi and Ren, Haoxing and Fang, Shao-Yun and Chen, Yiran and Hu, Jiang},
  booktitle={International Conference on Computer-Aided Design (ICCAD)},
  year={2018},
}

@inproceedings{krizhevsky2012imagenet,
  title={ImageNet Classification with Deep Convolutional Neural Networks},
  author={Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  booktitle={NIPS},
  year={2012}
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

@inproceedings{long2015fully,
  title={Fully convolutional networks for semantic segmentation},
  author={Long, Jonathan and Shelhamer, Evan and Darrell, Trevor},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={3431--3440},
  year={2015}
}

@inproceedings{lu2019nsga,
  title={Nsga-net: neural architecture search using multi-objective genetic algorithm},
  author={Lu, Zhichao and Whalen, Ian and Boddeti, Vishnu and Dhebar, Yashesh and Deb, Kalyanmoy and Goodman, Erik and Banzhaf, Wolfgang},
  booktitle={Proceedings of the Genetic and Evolutionary Computation Conference},
  pages={419--427},
  year={2019}
}

@inproceedings{lu2020nsganetv2,
  title={Nsganetv2: Evolutionary multi-objective surrogate-assisted neural architecture search},
  author={Lu, Zhichao and Deb, Kalyanmoy and Goodman, Erik and Banzhaf, Wolfgang and Boddeti, Vishnu Naresh},
  booktitle={European Conference on Computer Vision},
  pages={35--51},
  year={2020},
  organization={Springer}
}

@inproceedings{YuDAC19,
	author = "C. Yu and Z. Zhang", 
	title = "Painting on placement: forecasting routing congestion using conditional generative adversarial nets",
	booktitle = "ACM/IEEE Design Automation Conference",
	year = 2019} 	

@inproceedings{TabriziDAC18,
	author = "A.~F. Tabrizi and N.~K. Darav and S. Xu and L. Rakai and I. Bustany and A. Kennings and L. Behjat", 
	title = "A machine learning framework to identify detailed routing short violations from a placed netlist",
	booktitle = "ACM/IEEE Design Automation Conference",
	year = 2018} 	


@inproceedings{ChanISPD17,
	author = "W.-T. J. Chan and P.-H. Ho and A.~B. Kahng and P. Saxena", 
	title = "Routability optimization for industrial designs at sub-14nm process nodes using machine learning",
	page = {15-21},
	booktitle = "ACM International Symposium on Physical Design",
	year = 2017} 
	
@inproceedings{LiangISPD20,
  title={{DRC} Hotspot Prediction at Sub-10nm Process Nodes Using Customized Convolutional Network},
  author={R. Liang and H. Xiang and D. Pandey and L. Reddy and S. Ramji and G.-J. Nam and J. Hu},
  booktitle= "ACM International Symposium on Physical Design",
  year={2020}
}

@inproceedings{yu2019pin,
  title={Pin accessibility prediction and optimization with deep learning-based pin pattern recognition},
  author={Yu, Tao-Chun and Fang, Shao-Yun and Chiu, Hsien-Shih and Hu, Kai-Shun and Tai, Philip Hui-Yuh and Shen, Cindy Chin-Fang and Sheng, Henry},
  booktitle={Proceedings of the 56th Annual Design Automation Conference 2019},
  pages={1--6},
  year={2019}
}

@inproceedings{chen2020pros,
  title={{PROS}: A Plug-in for Routability Optimization applied in the State-of-the-art commercial {EDA} tool using deep learning},
  author={Chen, Jingsong and Kuang, Jian and Zhao, Guowei and Huang, Dennis J-H and Young, Evangeline FY},
  booktitle={2020 IEEE/ACM International Conference On Computer Aided Design (ICCAD)},
  pages={1--8},
  year={2020},
  organization={IEEE}
}

@article{hanley1982meaning,
  title={The meaning and use of the area under a receiver operating characteristic (ROC) curve.},
  author={Hanley, James A and McNeil, Barbara J},
  journal={Radiology},
  volume={143},
  number={1},
  pages={29--36},
  year={1982}
}

@inproceedings{deb2000fast,
  title={A fast elitist non-dominated sorting genetic algorithm for multi-objective optimization: NSGA-II},
  author={Deb, Kalyanmoy and Agrawal, Samir and Pratap, Amrit and Meyarivan, Tanaka},
  booktitle={International conference on parallel problem solving from nature},
  pages={849--858},
  year={2000},
  organization={Springer}
}

@inproceedings{deb2007self,
  title={Self-adaptive simulated binary crossover for real-parameter optimization},
  author={Deb, Kalyanmoy and Sindhya, Karthik and Okabe, Tatsuya},
  booktitle={Proceedings of the 9th annual conference on Genetic and evolutionary computation},
  pages={1187--1194},
  year={2007}
}

@article{cheng2019swiftnet,
  title={SwiftNet: Using Graph Propagation as Meta-knowledge to Search Highly Representative Neural Architectures},
  author={Cheng, Hsin-Pai and Zhang, Tunhou and Yang, Yukun and Yan, Feng and Li, Shiyu and Teague, Harris and Li, Hai and Chen, Yiran},
  journal={arXiv preprint arXiv:1906.08305},
  year={2019}
}

@inproceedings{alawieh2020high,
  title={High-definition routing congestion prediction for large-scale FPGAs},
  author={Alawieh, Mohamed Baker and Li, Wuxi and Lin, Yibo and Singhal, Love and Iyer, Mahesh A and Pan, David Z},
  booktitle={2020 25th Asia and South Pacific Design Automation Conference (ASP-DAC)},
  pages={26--31},
  year={2020},
  organization={IEEE}
}

@article{pham2018efficient,
  title={Efficient neural architecture search via parameter sharing},
  author={Pham, Hieu and Guan, Melody Y and Zoph, Barret and Le, Quoc V and Dean, Jeff},
  journal={arXiv preprint arXiv:1802.03268},
  year={2018}
}

@inproceedings{zoph2018learning,
  title={Learning transferable architectures for scalable image recognition},
  author={Zoph, Barret and Vasudevan, Vijay and Shlens, Jonathon and Le, Quoc V},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={8697--8710},
  year={2018}
}

@article{cai2018proxylessnas,
  title={Proxylessnas: Direct neural architecture search on target task and hardware},
  author={Cai, Han and Zhu, Ligeng and Han, Song},
  journal={arXiv preprint arXiv:1812.00332},
  year={2018}
}

@article{miller1995genetic,
  title={Genetic algorithms, tournament selection, and the effects of noise},
  author={Miller, Brad L and Goldberg, David E and others},
  journal={Complex systems},
  volume={9},
  number={3},
  pages={193--212},
  year={1995},
  publisher={[Champaign, IL, USA: Complex Systems Publications, Inc., c1987-}
}

################################## Manual

@manual{URL:IWLSbenchmarks,
  title   = "IWLS 2005 Benchmarks",
  address = "https://iwls.org/iwls2005/benchmarks.html"
}

@manual{URL:NanGate,
  title   = "NanGate 45nm Open Cell Library",
  address = "https://si2.org/open-cell-library/"
}

@manual{URL:ISPD15,
  title   = "ISPD 2015 Blockage-Aware Detailed Routing-Driven Placement Contest",
  address = "http://www.ispd.cc/contests/15/ispd2015\_contest.html"
}


@inproceedings{albrecht2005iwls,
  title={IWLS 2005 benchmarks},
  author={Albrecht, Christoph},
  booktitle={International Workshop for Logic Synthesis (IWLS): http://www. iwls. org},
  year={2005}
}


@inproceedings{bustany2015ispd,
  title={ISPD 2015 benchmarks with fence regions and routing blockages for detailed-routing-driven placement},
  author={Bustany, Ismail S and Chinnery, David and Shinnerl, Joseph R and Yutsis, Vladimir},
  booktitle={Proceedings of the 2015 Symposium on International Symposium on Physical Design},
  pages={157--164},
  year={2015}
}




@article{li2007routability,
  title={Routability-driven placement and white space allocation},
  author={Li, Chen and Xie, Min and Koh, Cheng-Kok and Cong, Jason and Madden, Patrick H},
  journal={IEEE Transactions on Computer-aided design of Integrated Circuits and Systems},
  volume={26},
  number={5},
  pages={858--871},
  year={2007},
  publisher={IEEE}
}

@inproceedings{tan2019mnasnet,
  title={Mnasnet: Platform-aware neural architecture search for mobile},
  author={Tan, Mingxing and Chen, Bo and Pang, Ruoming and Vasudevan, Vijay and Sandler, Mark and Howard, Andrew and Le, Quoc V},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={2820--2828},
  year={2019}
}

@article{abadi2016tensorflow,
  title={Tensorflow: Large-scale machine learning on heterogeneous distributed systems},
  author={Abadi, Mart{\'\i}n and Agarwal, Ashish and Barham, Paul and Brevdo, Eugene and Chen, Zhifeng and Citro, Craig and Corrado, Greg S and Davis, Andy and Dean, Jeffrey and Devin, Matthieu and others},
  journal={arXiv preprint arXiv:1603.04467},
  year={2016}
}

@article{pymoo,
    author={J. {Blank} and K. {Deb}},
    journal={IEEE Access},
    title={Pymoo: Multi-Objective Optimization in Python},
    year={2020},
    volume={8},
    pages={89497-89509},
}

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

@article{ramachandran2017searching,
  title={Searching for activation functions},
  author={Ramachandran, Prajit and Zoph, Barret and Le, Quoc V},
  journal={arXiv preprint arXiv:1710.05941},
  year={2017}
}

@inproceedings{liu2019auto,
  title={Auto-deeplab: Hierarchical neural architecture search for semantic image segmentation},
  author={Liu, Chenxi and Chen, Liang-Chieh and Schroff, Florian and Adam, Hartwig and Hua, Wei and Yuille, Alan L and Fei-Fei, Li},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={82--92},
  year={2019}
}

@article{chen2017rethinking,
  title={Rethinking atrous convolution for semantic image segmentation},
  author={Chen, Liang-Chieh and Papandreou, George and Schroff, Florian and Adam, Hartwig},
  journal={arXiv preprint arXiv:1706.05587},
  year={2017}
}

@article{tan2019mixconv,
  title={Mixconv: Mixed depthwise convolutional kernels},
  author={Tan, Mingxing and Le, Quoc V},
  journal={arXiv preprint arXiv:1907.09595},
  year={2019}
}


@inproceedings{qi2014accurate,
  title={Accurate prediction of detailed routing congestion using supervised data learning},
  author={Qi, Zhongdong and Cai, Yici and Zhou, Qiang},
  booktitle={2014 IEEE 32nd International Conference on Computer Design (ICCD)},
  pages={97--103},
  year={2014},
  organization={IEEE}
}


@inproceedings{chan2016beol,
  title={BEOL stack-aware routability prediction from placement using data mining techniques},
  author={Chan, Wei-Ting J and Du, Yang and Kahng, Andrew B and Nath, Siddhartha and Samadi, Kambiz},
  booktitle={2016 IEEE 34th International Conference on Computer Design (ICCD)},
  pages={41--48},
  year={2016},
  organization={IEEE}
}



@misc{Innovus,
  author = {Cadence},
  title = {Innovus Implementation System},
  url = {https://www.cadence.com/en_US/home/tools/digital-design-and-signoff/soc-implementation-and-floorplanning/innovus-implementation-system.html},
  year = {2021},
}

@inproceedings{brglez1989combinational,
  title={Combinational profiles of sequential benchmark circuits},
  author={Brglez, Franc and Bryan, David and Kozminski, Krzysztof},
  booktitle={IEEE International Symposium on Circuits and Systems (ISCAS)},
  pages={1929--1934},
  year={1989},
  organization={IEEE}
}




@article{corno2000rt,
  title={RT-level ITC'99 benchmarks and first ATPG results},
  author={Corno, Fulvio and Reorda, Matteo Sonza and Squillero, Giovanni},
  journal={Design \& Test of computers},
  year={2000},
}



@article{iandola2014densenet,
  title={Densenet: Implementing efficient convnet descriptor pyramids},
  author={Iandola, Forrest and Moskewicz, Matt and Karayev, Sergey and Girshick, Ross and Darrell, Trevor and Keutzer, Kurt},
  journal={arXiv preprint arXiv:1404.1869},
  year={2014}
}





@inproceedings{yang2021attacking,
  title={Attacking a {CNN}-based Layout Hotspot Detector Using Group Gradient Method},
  author={Yang, Haoyu and Zhang, Shifan and Liu, Kang and Liu, Siting and Tan, Benjamin and Karri, Ramesh and Garg, Siddharth and Yu, Bei and Young, Evangeline FY},
  booktitle={2021 26th Asia and South Pacific Design Automation Conference (ASP-DAC)},
  pages={885--891},
  year={2021},
  organization={IEEE}
}

@article{liu2020adversarial,
  title={{Adversarial perturbation attacks on ML-based CAD: A case study on CNN-based lithographic hotspot detection}},
  author={Liu, Kang and Yang, Haoyu and Ma, Yuzhe and Tan, Benjamin and Yu, Bei and Young, Evangeline FY and Karri, Ramesh and Garg, Siddharth},
  journal={ACM Transactions on Design Automation of Electronic Systems (TODAES)},
  year={2020},
}

@inproceedings{moosavi2019robustness,
  title={Robustness via curvature regularization, and vice versa},
  author={Moosavi-Dezfooli, Seyed-Mohsen and Fawzi, Alhussein and Uesato, Jonathan and Frossard, Pascal},
  booktitle={IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  year={2019}
}

@article{yang2018layout,
  title={Layout hotspot detection with feature tensor generation and deep biased learning},
  author={Yang, Haoyu and Su, Jing and Zou, Yi and Ma, Yuzhe and Yu, Bei and Young, Evangeline FY},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems (TCAD)},
  year={2018},
}

@article{rostami2014primer,
  title={A primer on hardware security: Models, methods, and metrics},
  author={Rostami, Masoud and Koushanfar, Farinaz and Karri, Ramesh},
  journal={Proceedings of the IEEE},
  year={2014},
  publisher={IEEE}
}

@article{madry2017towards,
  title={Towards deep learning models resistant to adversarial attacks},
  author={Madry, Aleksander and Makelov, Aleksandar and Schmidt, Ludwig and Tsipras, Dimitris and Vladu, Adrian},
  journal={arXiv preprint arXiv:1706.06083},
  year={2017}
}

@article{goodfellow2014explaining,
  title={Explaining and harnessing adversarial examples},
  author={Goodfellow, Ian J and Shlens, Jonathon and Szegedy, Christian},
  journal={arXiv preprint arXiv:1412.6572},
  year={2014}
}

@incollection{kurakin2018adversarial,
  title={Adversarial examples in the physical world},
  author={Kurakin, Alexey and Goodfellow, Ian J and Bengio, Samy},
  booktitle={Artificial intelligence safety and security},
  year={2018},
  publisher={Chapman and Hall/CRC}
}

@article{liu2016delving,
  title={Delving into transferable adversarial examples and black-box attacks},
  author={Liu, Yanpei and Chen, Xinyun and Liu, Chang and Song, Dawn},
  journal={arXiv preprint arXiv:1611.02770},
  year={2016}
}

@inproceedings{fawzi2018empirical,
  title={Empirical study of the topology and geometry of deep networks},
  author={Fawzi, Alhussein and Moosavi-Dezfooli, Seyed-Mohsen and Frossard, Pascal and Soatto, Stefano},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition},
  year={2018}
}

@article{jetley2018friends,
  title={With friends like these, who needs adversaries?},
  author={Jetley, Saumya and Lord, Nicholas and Torr, Philip},
  journal={Advances in neural information processing systems},
  volume={31},
  year={2018}
}

@inproceedings{reddy2018enhanced,
  title={Enhanced hotspot detection through synthetic pattern generation and design of experiments},
  author={Reddy, Gaurav Rajavendra and Xanthopoulos, Constantinos and Makris, Yiorgos},
  booktitle={VLSI Test Symposium (VTS)},
  year={2018}
}

@inproceedings{matsunawa2015new,
  title={A new lithography hotspot detection framework based on AdaBoost classifier and simplified feature extraction},
  author={Matsunawa, Tetsuaki and Gao, Jhih-Rong and Yu, Bei and Pan, David Z},
  booktitle={Design-Process-Technology Co-optimization for Manufacturability IX},
  volume={9427},
  year={2015},
  organization={SPIE}
}

@article{biggio2018wild,
  title={Wild patterns: Ten years after the rise of adversarial machine learning},
  author={Biggio, Battista and Roli, Fabio},
  journal={Pattern Recognition},
  volume={84},
  year={2018},
  publisher={Elsevier}
}

@inproceedings{deng2007coupling,
  title={Coupling-aware dummy metal insertion for lithography},
  author={Deng, Liang and Wong, Martin DF and Chao, Kai-Yuan and Xiang, Hua},
  booktitle={2007 Asia and South Pacific Design Automation Conference},
  year={2007},
  organization={IEEE}
}

@article{geng2019sraf,
  title={SRAF insertion via supervised dictionary learning},
  author={Geng, Hao and Zhong, Wei and Yang, Haoyu and Ma, Yuzhe and Mitra, Joydeep and Yu, Bei},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
  volume={39},
  number={10},
  year={2019},
  publisher={IEEE}
}

@inproceedings{otto1994automated,
  title={Automated optical proximity correction: a rules-based approach},
  author={Otto, Oberdan W and Garofalo, Joseph G and Low, KK and Yuan, Chi-Min and Henderson, Richard C and Pierrat, Christophe and Kostelak, Robert L and Vaidya, Sheila and Vasudev, PK},
  booktitle={Optical/Laser Microlithography VII},
  volume={2197},
  year={1994},
  organization={International Society for Optics and Photonics}
}

@inproceedings{xu2016machine,
  title={A machine learning based framework for sub-resolution assist feature generation},
  author={Xu, Xiaoqing and Matsunawa, Tetsuaki and Nojima, Shigeki and Kodama, Chikaaki and Kotani, Toshiya and Pan, David Z},
  booktitle={International Symposium on Physical Design (ISPD)},
  year={2016}
}

@inproceedings{yu2018developing,
  title={Developing synthesis flows without human knowledge},
  author={Yu, Cunxi and Xiao, Houping and De Micheli, Giovanni},
  booktitle={Design Automation Conference (DAC)},
  year={2018}
}

@inproceedings{kahng2018machine,
  title={Machine learning applications in physical design: Recent results and directions},
  author={Kahng, Andrew B},
  booktitle={International Symposium on Physical Design (ISPD)},
  year={2018}
}

@article{rapp2021mlcad,
  title={{MLCAD}: A Survey of Research in Machine Learning for {CAD} Keynote Paper},
  author={Rapp, Martin and Amrouch, Hussam and Lin, Yibo and Yu, Bei and Pan, David Z and Wolf, Marilyn and Henkel, J{\"o}rg},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems (TCAD)},
  year={2021},
  publisher={IEEE}
}

@article{xie2022dark,
  title={The Dark Side: Security Concerns in Machine Learning for EDA},
  author={Xie, Zhiyao and Pan, Jingyu and Chang, Chen-Chia and Hu, Jiang  and Chen, Yiran},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems (TCAD)},
  year={2022},
}


@misc{graphics2008calibre,
  title={Calibre verification user’s manual},
  author={Graphics, Mentor},
  year={2008}
}

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

@inproceedings{nair2010rectified,
  title={Rectified linear units improve restricted boltzmann machines},
  author={Nair, Vinod and Hinton, Geoffrey E},
  booktitle={Icml},
  year={2010}
}


@inproceedings{zhang2016enabling,
  title={Enabling online learning in lithography hotspot detection with information-theoretic feature optimization},
  author={Zhang, Hang and Yu, Bei and Young, Evangeline FY},
  booktitle={International Conference on Computer-Aided Design (ICCAD)},
  year={2016},
}




@article{yang2017imbalance,
  title={Imbalance aware lithography hotspot detection: a deep learning approach},
  author={Yang, Haoyu and Luo, Luyang and Su, Jing and Lin, Chenxi and Yu, Bei},
  journal={Journal of Micro/Nanolithography, MEMS, and MOEMS},
  year={2017},
}


@article{yang2021vlsi,
  title={{VLSI} mask optimization: From shallow to deep learning},
  author={Yang, Haoyu and Zhong, Wei and Ma, Yuzhe and Geng, Hao and Chen, Ran and Chen, Wanli and Yu, Bei},
  journal={Integration},
  year={2021},
  publisher={Elsevier}
}


@inproceedings{reddy2019machine,
  title={Machine learning-based hotspot detection: Fallacies, pitfalls and marching orders},
  author={Reddy, Gaurav Rajavendra and Madkour, Kareem and Makris, Yiorgos},
  booktitle={International Conference on Computer-Aided Design (ICCAD)},
  year={2019},
}

@inproceedings{liu2020poisoning,
  title={Poisoning the (data) well in {ML-based CAD}: A case study of hiding lithographic hotspots},
  author={Liu, Kang and Tan, Benjamin and Karri, Ramesh and Garg, Siddharth},
  booktitle={Design, Automation \& Test in Europe Conference \& Exhibition (DATE)},
  year={2020},
}


@inproceedings{torres2012iccad,
  title={{ICCAD-2012 CAD} contest in fuzzy pattern matching for physical verification and benchmark suite},
  author={Torres, J Andres},
  booktitle={International Conference on Computer-Aided Design (ICCAD)},
  year={2012},
}

@inproceedings{ribeiro2016should,
  title={"{Why should I trust you?" Explaining the predictions of any classifier}},
  author={Ribeiro, Marco Tulio and Singh, Sameer and Guestrin, Carlos},
  booktitle={International Conference on Knowledge Discovery and Data Mining (KDD)},
  year={2016}
}




@inproceedings{pan2022robustify,
  title={Robustify ML-Based Lithography Hotspot Detectors},
  author={Pan, Jingyu and Chang, Chen-Chia and Xie, Zhiyao and Hu, Jiang and Chen, Yiran},
  booktitle={International Conference on Computer-Aided Design (ICCAD)},
  year={2022},
}


@article{linardatos2020explainable,
  title={Explainable {AI}: A review of machine learning interpretability methods},
  author={Linardatos, Pantelis and Papastefanopoulos, Vasilis and Kotsiantis, Sotiris},
  journal={Entropy},
  year={2020},
  publisher={MDPI}
}



@article{scikit-learn,
 title={{Scikit-learn: Machine Learning in Python}},
 author={Pedregosa, Fabian and Varoquaux, Ga{\"e}l and Gramfort, Alexandre and Michel, Vincent and Thirion, Bertrand and Grisel, Olivier and Blondel, Mathieu and Prettenhofer, Peter and Weiss, Ron and Dubourg, Vincent and others},
 journal={JMLR},
 year={2011}
}

@article{paszke2019pytorch,
  title={{PyTorch}: An Imperative Style, High-Performance Deep Learning Library},
  author={Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and others},
  journal={Neural Information Processing Systems (NeurIPs)},
  year={2019}
}




